Empirical Analysis of Near-Field Beam Shaping for Blockage Events

Millimeter-wave (mmWave) to sub-terahertz (sub-THz) links can realize high data rates, yet are highly vulnerable to dynamic blockages due to high directivity, limited multipath, and dependence on line-of-sight (LoS) propagation. While structured and self-healing beams are promising solutions, it remains unclear how beam types perform under dynamic blockage. In this paper, we present an empirical analysis of structured near-field beams using two transmission policies. At one extreme, we study beam resilience without obstacle adaptation. At the other extreme, we empirically optimize beam parameters to study the limits of multiple beam types under idealized adaptation. We employ numerical analysis based on the angular spectrum method (ASM) and experimental validation using a sub-THz time-domain spectroscopy (TDS) platform to characterize beam performance over complete blockage events. For the scenarios considered, despite lacking self-healing, focused beams provide the strongest resilience when beam parameters are not adapted during a blockage event (i.e., when all beams are optimized only a priori). In contrast, when optimally adapted to obstacle position, curved beams provide the best performance. Lastly, although Bessel beams benefit from self-healing, this property alone can be insufficient to outperform optimized curved and focused beams. These findings provide guidance for blockage-aware beam selection and adaptation protocols.

==> experiment.tex <==
\section{Experimental Results}



==> fundamentals.tex <==
\section{System Model and Beam Shape Generation}
% In this section, we establish the near-field system model, define the four canonical beam shapes in our toolbox, and introduce the exact wave propagation models used to evaluate dynamic blockage events.

This section defines the near-field link geometry, dynamic blockage-event model, beam-shaping toolbox, and wave-propagation method used throughout the paper. The objective is to create a common modeling framework in which different beam shapes and adaptation policies can be compared under identical blockage conditions.

\subsection{Coordinate System}
We consider a sub-THz near-field communication system operating at a center frequency $f_c$. At these high frequencies, the electrically large size of the transmitting aperture significantly extends the near-field (Fresnel) region, allowing us to exploit non-planar wavefronts for advanced beam shaping \cite{singh2023wavefront}.

Consider the access point (AP) equipped with a uniform linear array (ULA) to serve a static user with a single antenna, as shown in Fig.\ref{fig:system-model}. We define the system within a 2D Cartesian coordinate system (xz-plane). The ULA is centered at the origin along the x-axis and consists of $N$ elements separated by a uniform spacing $d$. This yields a total physical aperture size of $D=(N-1)d$. The coordinate of the $n$-th element is therefore given by $x_n=(n-\frac{N-1}{2})d$. The desired phase profile of the considered beam shape for the near-field beam is applied across the $x_n$ elements. The user equipment (UE) is located at a fixed spatial target with coordinates $(x_u,z_u)$, where $x_u$ denotes the transverse position and $z_u$ denotes the longitudinal distance along the propagation axis.

Due to obstacles in the propagation environment, which can easily disrupt communication, we model dynamic Line-of-Sight (LoS) blockages as time-varying objects moving transversely across the propagation link. Because the engineered near-field beams have highly narrow beamwidths \cite{bodet2024sub}, the probability that a dynamic object experiences significant longitudinal displacement while actively crossing the beam's core is exceptionally low. As a result, we can simplify the blockage trajectory as passing perpendicularly through the propagation axis at a fixed intermediate depth $z_b$, ignoring any negligible depth variations ($\Delta z$) during the crossing event. To systematically analyze the impact of these dynamic events, we define the blockage width, $W_b$, as a fractional ratio of the transmitting aperture size $D$. Specifically, we evaluate the system under various blockage severities where $W_b \in \{\frac{1}{8}D, \frac{1}{4}D, \frac{1}{2}D, D\}$.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/.png}
    \caption{Modeled deployment scenario.}
    \label{fig:system-model}
\end{figure}

\begin{figure*}[t]
    \centering
    % Subfigure 1
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gaussian-example.pdf}
        \caption{Gaussian beam}
        \label{fig:row1}
    \end{subfigure}
    \hfill % This adds horizontal space between the images
    % Subfigure 2
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/focused-example.pdf}
        \caption{Focused beam}
        \label{fig:row2}
    \end{subfigure}
    \hfill
    % Subfigure 3
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/bessel-example.pdf}
        \caption{Bessel beam}
        \label{fig:row3}
    \end{subfigure}
    \hfill
    % Subfigure 4
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/curved-example.pdf}
        \caption{Curved beam}
        \label{fig:row4}
    \end{subfigure}

    \caption{The proposed near-field beam shaping toolbox.}
    \label{fig:beam-shaping-toolbox}
\end{figure*}

\subsection{Beam Shape Generation}
To address the diverse, highly variable nature of dynamic near-field blockages, our framework leverages a comprehensive \textit{Beam Shaping Toolbox}. Instead of relying on a single transmission strategy, we evaluate four canonical beam designs: Gaussian, Focused, Bessel, and Curved. Each beam shape exhibits unique propagation characteristics and requires a distinct phase profile, denoted as $\phi_n)$, applied across the discrete elements of the ULA. Fig. \ref{fig:beam-shaping-toolbox} presents the normalized intensity of the E-field from different beams.

\textbf{Gaussian Beam:} This serves as the standard directional beam steered toward a specific angle $\theta$. The linear phase profile applied to the $n$-th element to steer the beam is given by
\begin{equation}
        \phi_{n,\text{Gaussian}}(\theta) = -2\pi f_c x_n \sin\theta.
\end{equation}

\textbf{Focused Beam:} Unlike standard steering, a focused beam engineers a hyperboloidal wavefront designed to concentrate its energy at a specific focal length $l$ along the propagation axis \cite{nepa2017near, liao2025terafocus}. The required non-linear phase profile to focus the beam at depth $l$ while steering at angle $\theta$ is given by
\begin{equation}
        \phi_{n, \text{Focused}}(\theta, l) = 2\pi f_c \left(\sqrt{x_n^2+l^2} - l - x_n\sin\theta\right).
\end{equation}

\textbf{Bessel Beam:} Bessel beams are non-diffracting wavefronts characterized by a central energy core surrounded by concentric rings \cite{durnin1988comparison, reddy2023ultrabroadband}. The required phase profile is dictated by the deflection angle $\psi_b$, which controls the inward interference pattern. To generate this structure while simultaneously steering the beam toward an azimuth angle $\theta$, the required phase profile is given by
\begin{equation}
    \phi_{n, \text{Bessel}}(\theta, \psi_b) = 2\pi f_c \left(|x_n| \sin\psi_b - x_n\sin\theta\right).
\end{equation}
    
\textbf{Curved Beam (Caustics):} A phase-only caustic beam is designed to follow a continuous spatial trajectory, typically defined by the function $g(z)$ \cite{guerboukha2024curving}. As illustrated in Fig. \ref{fig:curved-trajectory}, this allows the caustic envelope to systematically bend around potential LoS blockages before smoothly converging at the intended spatial target. To evaluate this obstacle avoidance capability alongside standard steering and focusing, our framework explicitly parameterizes the physical path as a cubic polynomial, $g(z;\theta,l,\kappa)$. As detailed in Appendix A, this setup uses the focal distance $l$ and steering angle $\theta$ to define the beam's exact target, while the curvature parameter $\kappa$ independently controls how sharply the beam bends. To bypass blockages from either side of the direct path, a phase-inversion mapping is applied to mirror the trajectory across the propagation axis. The absolute phase profile for the $n$-th element is determined by integrating the continuous phase derivative across the aperture, which is expressed as
\begin{equation}
    \phi_{n, \text{Curved}}(\theta, l, \kappa) = 2\pi f_c \int_{0}^{x_n} \left( \frac{g'(z)}{\sqrt{1+g'(z)^2}} - \sin\theta \right) dx.
\end{equation}

% \begin{figure}[b]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/curved-trajectory.pdf}
%     \caption{Trajectory of the Curved beam.}
%     \label{fig:curved-trajectory}
% \end{figure}


\subsection{Near-Field Wave Propagation and Blockage Modeling}
Once the discrete phase profile $\phi_n$ is applied to the ULA to synthesize the desired beam shape, its propagation through the near-field channel must be accurately modeled in the presence of dynamic obstructions. Conventional geometric channel models, such as standard ray-tracing approximations, are fundamentally inadequate in this regime as they fail to capture the complex diffraction and interference phenomena that occur when sub-THz waves interact with finite obstacles. Moreover, the computational overhead of full-wave EM simulators makes them impractical for thorough parameter sweeps needed to find optimal beam configurations.

To overcome these limitations, we utilize the Angular Spectrum Method (ASM) \cite{yazdnian2025nirvawave} to compute the exact near-field E-field distribution. The ASM provides an exact, scalar solution to wave propagation by recasting the Rayleigh-Sommerfeld diffraction integral \cite{born2013principles} into the spatial Fourier domain. Let $E(x,0)$ denote the initial complex E-field at the transmitter aperture. The E-field at any arbitrary longitudinal distance $z$ is calculated by
\begin{align}
    E(x,z)=\mathcal{F}^{-1}\{\mathcal{F}\{E(x,0)\}\cdot H(k_x, z)\}.
\end{align}
where $H(k_x,z)=\exp{jz\sqrt{k^2-k_x^2}}$ represents the free-space transfer function.

To model a dynamic blockage event, we evaluate the propagation in two distinct stages. The wave first propagates to an intermediate distance $z_b$ where the obstacle is situated, yielding the incident field $E(x,z_b)$. At this transverse plane, we apply a spatial interaction mask, $M(x)$, defined as
\begin{align}
        M(x) = \begin{cases} 
      \Gamma, & \text{if } x \in W_b \\ 
      1, & \text{otherwise} 
   \end{cases}
\end{align}
where $\Gamma$ is a complex coefficient that characterizes the material properties of the blockage. For a perfectly absorbing obstacle, $\Gamma=0$ effectively nullifies the E-field components intersecting the blockage. Conversely, for a reflecting blockage, $\Gamma$ serves as a reflection coefficient that scales the incident field magnitude to account for material-specific losses.

Consistent with the recursive logic of our simulation, this reflected component is treated as a secondary source and re-propagated through the environment, while the unblocked portion of the field continues toward the receiver. Finally, by calculating the total E-field distribution $E(x_u,z_u)$ arriving at the user's coordinates $(x_u, z_u)$, we can integrate the intensity across the receiver's aperture to determine the total received signal power as the mask dynamically traverses the link.
